Mechanisms for Trading Durable Goods

We consider trading indivisible and easily transferable \emph{durable goods}, which are goods that an agent can receive, use, and trade again for a different good. This is often the case with books that can be read and later exchanged for unread ones. Other examples of such easily transferable durable goods include puzzles, video games and baby clothes. We introduce a model for the exchange of easily transferable durable goods. In our model, each agent owns a set of items and demands a different set of items. An agent is interested in receiving as many items as possible from his demand set. We consider mechanisms that exchange items in cycles in which each participating agent receives an item that he demands and gives an item that he owns. We aim to develop mechanisms that have the following properties: they are \emph{efficient}, in the sense that they maximize the total number of items that agents receive from their demand set, they are \emph{strategyproof} (i.e., it is in the agents' best interest to report their preferences truthfully) and they run in \emph{polynomial time}. One challenge in developing mechanisms for our setting is that the supply and demand sets of the agents are updated after a trade cycle is executed. This makes constructing strategyproof mechanisms in our model significantly different from previous works, both technically and conceptually and requires developing new tools and techniques. We prove that simultaneously satisfying all desired properties is impossible and thus focus on studying the tradeoffs between these properties. To this end, we provide both approximation algorithms and impossibility results.

==> Extensions.tex <==
\section{Extension of the Agent's Utility Function} \label{utility-extensions}
So far we assumed that an agent has a very high cost (i.e., $\sum_{i=1}^n| D_i |$) for receiving an item that is not in his demand set. In this section we relax this assumption and instead assume that the cost of agent $i$ of receiving an item that is not in $D_i$ is $c < \sum_{i=1}^n |D_i |$. Formally, we define the \emph{generalized} utility function of an agent $i$ in execution $r$ as:
$\hat u_i(r) = |D_i\cap A_i(r)|- c \cdot |A_i(r)\setminus D_i|.$

For $c=\sum_{i=1}^n| D_i |$ any execution that maximizes the social welfare cannot allocate any agent an item that he does not demand as this will result in negative social welfare. This is no longer the case when we consider smaller values of $c$. As a result, there are instances in which the optimal execution is not individually rational and an agent can benefit by not reporting all the items that he owns:
  
\begin{proposition}\label{prop:utility}
For agents with generalized utility functions and $0< c < \sum_{i=1}^n |D_i |$, any strategyproof algorithm cannot guarantee a finite approximation ratio. 
\end{proposition}
\begin{proof}
Consider a trading graph which has a path that begins with item $j$ and ends with an agent $a$. The optimal execution $r$ in this instance will allocate each agent in the path the item that he demands and agent $a$ is allocated item $j$. The social welfare of this execution is $\sum_i \hat u_i(r)=\sum_{i=1}^n |D_i| - c$ which is positive since $c<\sum_{i=1}^n |D_i|$. However, the utility of agent $a$ is negative. In general,  observe that any execution has to include an agent that has a negative utility because he receives an item that he is not interested in. The agent with the negative utility can increase his utility to $0$ by not reporting the item he owns. Thus, we conclude that in this instance a strategyproof algorithm cannot make any exchanges at all and hence provides an unbounded approximation ratio to the optimal execution.
\end{proof}

The proposition motivates our choice of focusing on $c = \sum_{i=1}^n |D_i|$ as it shows that this is the minimal cost required to avoid those pathological impossibility results. In Appendix \ref{app-utility} we complete the picture by showing that the strategyproof algorithm that we presented in Section \ref{subsec:strategyproofness} for computing an optimal static execution is also 
 strategyproof with respect to the generalized utility functions: 
\begin{theorem} \label{thm:as-generzlied}
	The static algorithm $A_s$ described in Section \ref{subsec:strategyproofness} is strategyproof for agents with generalized utility functions and for any $c\geq 0$.
\end{theorem}

Note,  that there is no guarantee on the approximation ratio of $A_s$ with the generalized utility functions.
%that since the algorithm $A_s$ is strategyproof, by Proposition \ref{prop:utility} we have that there is no guarantee on the approximation ratio with the generalized utility functions. 
Moreover, as previously discussed, the utility function studied by Abbassi et al.  \cite{abbassi2015exchange} is similar to the generalized utility function defined above for $c=0$. Thus, Theorem \ref{thm:as-generzlied} proves the applicability of our algorithm to the setting of \cite{abbassi2015exchange}. %As discussed previously, our algorithm has the advantage that it allows the selection of more "fair" and balanced executions. 

